Completing the four-body contributions to $\bar{B}\rightarrow X_s \gamma$ at NLO

We report on the status of the ongoing calculation of multiparticle contributions to the inclusive radiative $\bar{B} \rightarrow X_s \gamma$ decay at next-to leading order. This effort amounts to the evaluation of the four-particle process $b\rightarrow s \bar{q} q \gamma$ at the one-loop level, supplemented by the corresponding five-particle tree-level cuts $b\rightarrow s \bar{q} q \gamma + g$ of the gluon bremsstrahlung. Knowledge of these pieces will formally complete the $\bar{B} \rightarrow X_s \gamma$ decay at the next-to-leading order. The different steps such as the generation of the amplitude, its renormalization, and the treatment of occurring IR-divergences are discussed. Moreover, we elaborate on the subtleties that arise when treating $\gamma_5$ in $D$ dimensions.

==> bibavignon.tex <==
\bibitem{huber:1411}
 \bibentry{{T. Huber, M. Poradziński and J. Virto}}
 {{Four-body contributions to $ \bar{B} \rightarrow {X}_s\gamma$ at NLO}}
 {\jhep{01}{2015}{115}}
 {\arxiv{1411.7677}{hep-ph}}
 
\bibitem{burasfierz05}
 \bibentry{{A. J. Buras, M. Misiak and J. Urban}}
 {{Two loop QCD anomalous dimensions of flavor changing
 four quark operators within and beyond the standard
 model}}
 {\npb{586}{2000}{397-426}}
 {\hepph{0005183}}
 
\bibitem{bsgth}
 \bibentry{{M. Misiak et al.}}
 {{Updated NNLO QCD predictions for the weak radiative B-meson decays}}
 {\prl{114}{2015}{221801}}
 {\arxiv{1503.01789}{hep-ph}}
 
\bibitem{bsgex}
 \bibentry{{HFLAV Collaboration}}
 {{Averages of $b$-hadron, $c$-hadron, and $\tau$-lepton properties as of summer 2016}}
 {{\epjc{77}{2017}{895}}}
 {\arxiv{1612.07233}{hep-ex}}
 
\bibitem{burasnlo}
 \bibentry{{A. J. Buras, A. Czarnecki, M. Misiak and J. Urban}}
 {{Completing the NLO QCD calculation of $\bar{B} \rightarrow X_S \gamma$)}}
 {\npb{631}{2002}{219-238}}
 {\hepph{0203135}}
 
\bibitem{misiak06}
 \bibentry{M. Misiak et al.}
 {{Estimate of $\mathcal{B} (\bar B \to X_s \gamma)$ at $O(\alpha_s^2)$}}
 {\prl{98}{2007}{022002}}
 {\hepph{0609232}}
 
\bibitem{misiak10}
 \bibentry{M. Misiak and M. Poradziński}
 {{Completing the Calculation of BLM corrections to $\bar{B}$ to $X_s \gamma$}}
 {\prd{83}{2011}{014024}}
 {\arxiv{1009.5685}{hep-ph}}
 
\bibitem{kam12}
 \bibentry{M. Kamiński, M. Misiak and M. Poradziński}
 {{Tree-level contributions to $B \rightarrow X_s \gamma$}}
 {\prd{86}{2012}{094004}}
 {\arxiv{1209.0965}{hep-ph}}

\bibitem{ps4}
 \bibentry{{A. Gehrmann-De Ridder, T. Gehrmann and G. Heinrich}}
 {{Four particle phase space integrals in massless QCD}}
 {\npb{682}{2004}{265-288}}
 {\hepph{0311276}}
 
\bibitem{ps5}
 \bibentry{{G. Heinrich}}
 {{Towards $e^+ e^- \rightarrow 3$ jets at NNLO by sector decomposition}}
 {\epjc{48}{2006}{25-33}}
 {\hepph{0601062}}
 
\bibitem{melnikovibp}
 \bibentry{{C. Anastasiou and K. Melnikov}}
 {{Higgs boson production at hadron colliders in NNLO QCD}}
 {\npb{646}{2002}{220-256}}
 {\hepph{0207004}}
 
\bibitem{feyncalc}
 \bibentry{V. Shtabovenko}
 {New Developments in FeynCalc 9.0}
 {\cpc{207}{2016}{432-444}}
 {\arxiv{1601.01167}{hep-ph}}

\bibitem{form}
 \bibentry{B. Ruijl, T. Ueda and J. Vermaseren}
 {FORM version 4.2}
 {\arxiv{2017}{hep-ph}}
 {}
 
\bibitem{fire}
 \bibentry{{A. V. Smirnov and F. S. Chuharev}}
 {{FIRE6: Feynman Integral REduction with Modular Arithmetic}}
 {\arxiv{1901.07808}{hep-ph}}
 {}
 
\bibitem{hypexp}
 \bibentry{T. Huber and D. Maitre}
 {HypExp 2, Expanding Hypergeometric Functions about Half-Integer Parameters}
 {\cpc{178}{2008}{755-776}}
 {\arxiv{0708.2443}{hep-ph}}

\bibitem{qgraf}
 \bibentry{P. Nogueira}
 {Automatica Feynman graph generation}
 {\jcp{105}{1993}{279}}
 {} 
 
